Mixed Integer Programming for Time-Optimal Multi-Robot Coverage Path Planning with Efficient Heuristics

We investigate time-optimal Multi-Robot Coverage Path Planning (MCPP) for both unweighted and weighted terrains, which aims to minimize the coverage time, defined as the maximum travel time of all robots. Specifically, we focus on a reduction from MCPP to Min-Max Rooted Tree Cover (MMRTC). For the first time, we propose a Mixed Integer Programming (MIP) model to optimally solve MMRTC, resulting in an MCPP solution with a coverage time that is provably at most four times the optimal. Moreover, we propose two suboptimal yet effective heuristics that reduce the number of variables in the MIP model, thus improving its efficiency for large-scale MCPP instances. We show that both heuristics result in reduced-size MIP models that remain complete (i.e., guaranteed to find a solution if one exists) for all MMRTC instances. Additionally, we explore the use of model optimization warm-startup to further improve the efficiency of both the original MIP model and the reduced-size MIP models. We validate the effectiveness of our MIP-based MCPP planner through experiments that compare it with two state-of-the-art MCPP planners on various instances, demonstrating a reduction in the coverage time by an average of 27.65% and 23.24% over them, respectively.

==> abstract.tex <==
\begin{abstract}
We study the time-optimal Multi-Robot Coverage Path Planning (MCPP) problem for both unweighted and weighted terrains, which aims to minimize the coverage time (i.e., makespan), defined as the maximum of the travel times of all robots.
We propose a Mixed Integer Programming (MIP) model based on the reduction from the MCPP problem to the Rooted Min-Max Tree Cover (RMMTC) problem, thereby solving the MCPP problem with the proof that the makespan is at most four times larger than the minimal.
In addition, we propose two efficient suboptimal heuristics to reduce the number of variables of the MIP model, thus improving its efficiency for large-scale MCPP problems.
Theoretically, we prove that the MIP model optimally solves RMMTC problems and that the reduced-size MIP models resulting from both heuristics remain complete for RMMTC problems.
Additionally, we explore the use of model optimization warm-startup to further improve the solving efficiencies of both the original MIP model and the reduced-size MIP models.
Experimentally, we showcase the effectiveness of our MIP-based MCPP planner through comparisons with two state-of-the-art MCPP planners on various instances, demonstrating an average reduction in the coverage time of $42.42\%$ and $39.16\%$ compared with MFC and MSTC$^*$, respectively. 
\end{abstract}

\begin{IEEEkeywords}
Planning, Multi-Robot System
\end{IEEEkeywords}



==> bcp.tex <==
\section{The Branch-Cut-and-Price Framework}
Following~\cite{barnhart1998branch}, we first reformulate the original RMMTC problem in Eqn.~(\ref{eqn:obj}) similar to the partitioning model with identical restrictions on subsets, since it exhibits a tight LP relaxation and eliminates symmetric structure.
We then adopt the Branch-Cut-and-Price (BCP) framework to solve the reformulated problem with a huge number of variables.
% \begin{figure}[htp]
% \centering
% \includegraphics[width=0.9\linewidth]{figs/Branch_and_price_diagram.png}
% \caption{Branch-and-Price Flow Diagram from Wiki.}
% \label{fig:bcp_diagram}
% \end{figure}
\subsection{The Master Problem}
For each $i\in I$, let $\mathcal{T}_i$ be a candidate tree pool for the $i$-th rooted subtree, then we define $\lambda_t\in[0, 1]$ as a continuous variable representing the proportion of using an arbitrary tree $t\in\mathcal{T}_i$ rooted at $r_i\in R$ as subtree $T_i$.
Within each tree $t\in\mathcal{T}_i$, we let $x_e^t$ and $y_v^t$ take values of $1$ if edge $e$ and vertex $v$ exist and $0$ otherwise, respectively.
We now define following Linear Programming (LP) problem as the Master Problem (MP):
\begin{align}
\label{bcp:obj}\textbf{(LP)}&\quad\displaystyle{\minimize_{\lambda, \tau}\quad\tau} &\\
\label{bcp:makespan}\text{s.t.}&\sum_{t\in \mathcal{T}_i}\sum_{e\in E} w_{e} x^t_{e} \lambda_t \leq \tau, &\forall i\in I\\
\label{bcp:cover}&\sum_{t\in \mathcal{T}_i}\sum_{i\in I} y^t_v\lambda_t\geq 1, &\forall v \in V\\
\label{bcp:convexity}&\sum_{t\in \mathcal{T}_i}\lambda_t=1, &\forall i\in I
\end{align}
where Eqn.~(\ref{bcp:makespan}) is the \textit{Makespan} constraint, Eqn.~(\ref{bcp:cover}) is the \textit{Cover} constraints, and Eqn.~(\ref{bcp:convexity}) is the convexity constraint that ensures each subtree uses exactly one tree.
The reformulation also brings advantages of removal of the \textit{Rooted} and \textit{Tree} constraints compared with the original MIP, as we have restricted our decision variables only on such valid trees.

\subsection{Cutting Planes}
Redundant heuristic constraints can be added dynamically when necessary to tighten the solution space, which are also known as the \textit{cutting planes}.

\subsection{The Pricing Subproblem}
The role of the Pricing Subproblem (PS) is to dynamically add new valid trees into the candidate tree pool $\mathcal{T}_i$ for $i\in I$, which would potentially improve the objective value.
For each $i\in I$ and $v\in V$, we denote $\alpha_i \leq 0$, $\beta_v \geq 0$ and $\gamma_i\in\mathbb{R}$ as the dual variables for the \textit{Makespan} constraints (\ref{bcp:makespan}), \textit{Cover} constraints (\ref{bcp:cover}) and convexity constraints (\ref{bcp:convexity}), respectively.
Based on the dual constraints with respect to each primal variable $\lambda_t$ where $i\in I, t\in \mathcal{T}_i$, the canonical reduced cost for the corresponding tree $t$ is given as below:
\begin{align*}
c_i(t):=\tau-\sum_{e\in E}\hat{\alpha_i}w_ex_e^t - \sum_{v\in V}\hat{\beta_v}y_v^t - \hat{\gamma_i}
\end{align*}
where $\hat{\alpha_i}$, $\hat{\beta_v}$ and $\hat{\gamma_i}$ are the current optimal dual solution.
The PS for each $i\in I$ is to find a tree (or trees) with strictly negative reduced cost (also known as the \textit{stability analysis}): a) if we have found a tree $t$ with $c_i(t)<0$, then $t$ would potentially improve the objective so we add $t$ into  $\mathcal{T}_i$;
b) if $\forall i\in I, c_i(t)\geq 0$, we can claim that the current solution is optimal for the MP~\cite{}.
We can intuitively interpret the PS as follows: compared with the current optimal solution, we try to find a tree with negative reduced cost that uses fewer edges (i.e. minimizing the second term) to cover more vertices (i.e. minimizing the third term) without violating the primal constraints.
Notice that since the first term $\tau\geq\sum_{e\in E}w_ex^t_e$, we can further derive a relaxed reduced cost $\bar{c_i}(t)$:
\begin{align}\label{bcp:relaxed_reduced_cost}
\bar{c_i}(t):=\sum_{e\in E}(1-\hat{\alpha_i})w_ex_e^t - \sum_{v\in V}\hat{\beta_v}y_v^t -\hat{\gamma_i}\leq c_i(t)
\end{align}

During each BCP pricing phase among all $i\in I$, there must exist one and only one \textit{bottleneck} $j\in I$ where $c_j(t)=\bar{c_j}(t)$, and $c_i(t)>\bar{c_i}(t)$ for all other \textit{non-bottlenecks} $i\in I/\{j\}$.
Therefore, if we apply the relaxed reduced cost in Eqn.~(\ref{bcp:relaxed_reduced_cost}) instead of the canonical one, the PS for the bottleneck would have the exact optimal solution, whereas the non-bottlenecks include not only the trees with $\bar{c_i}(t)<0$ but also some trees with $c_i(t)\geq 0$.
Fortunately, as the BCP framework iterates to the optimal, the difference between the weight of each subtree will be reduced a lot thus eliminating most of the unnecessary trees with $\bar{c_i}(t)<0$ but $c_i(t)\geq 0$.
Formally, we can write the PS for each $i\in I$ based on the relaxed reduced cost as the following minimization problem:
\begin{align*}
\min_t\;\bar{c_i}(t) = \min_t \left\{\sum_{e\in E}(1-\hat{\alpha_i})w_ex_e^t + \sum_{v\in V}-\hat{\beta_v}y_v^t\right\} -\hat{\gamma_i}
\end{align*}
which is actually equivalent to finding the minimum weighted (both vertex and edge weights) subtree rooted at $r_i\in R$ on the original graph $G$, with the vertex and edge weights replaced by $-\hat{\beta_v}$ and $(1-\hat{\alpha_i})w_e$.
Since $\alpha_i\leq 0$ and $\beta_v\geq 0$, the above vertex weight is negative and the above edge weight is positive.
The PS is similar to the k-MST problem which is NP-hard.


% Luckily, the above pricing subproblem can be solved optimally in polynomial time based on Prim's algorithm for Minimum Spanning Tree (MST).
% The modified Prim's algorithm for our problem is described in Algorithm~\ref{alg:pricing}.
% In the following, we prove its correctness on finding such minimum rooted weighted subtree.
% \begin{proof}
% Assume $T^*_k$ is the optimum (i.e. minimum vertex and edge weighted) subtree with $k$ vertices rooted at $r$.
% Clearly, the optimal subtree rooted at $r$ with an arbitrary number of vertices must be chosen from $T^*_1, T^*_2, ..., T^*_n$, where $n$ is the number of vertices of graph $G$.
% We further assume $M_k$ is the intermediate MST constructed from line~\ref{alg_pricing_line:intermediate} after $k$-th iteration, where $k=1,2,...,n$.
% Since the min heap $Q$ is ordered by the sum of vertex weight and its inducing edge weight (line~\ref{alg_pricing_line:enqueue}), we get the best possible vertex that can be grown from $M_{k-1}$ when $Q$ dequeues (line~\ref{alg_pricing_line:dequeue}) in the $k$-th iteration.
% It satisfies that the constructed $M_k$ must be the minimum $r$-rooted subtree with $k$ vertices, in other words, we obtain $M_k=T^*_k$.
% Therefore, the algorithm acquires the optimum subtree by updating the optimum with $M_k$ (line~\ref{alg_pricing_line:update_st}-\ref{alg_pricing_line:update_ed}) in each iteration until $n$ iterations.
% \end{proof}
% \begin{algorithm}
% \DontPrintSemicolon
% \caption{Modified Prim's Algorithm}\label{alg:pricing}
% \KwData{$G(V,E)$, $r\in V$, vertex weight $f(v)$, edge weight $g(e)$}
% \KwResult{minimum weighted subtree $T$ rooted at $r$}
% $S \gets \{\}$ \tcp*{visited vertex set}
% $F \gets \{\}$ \tcp*{edge set of current subtree}
% $Q \gets \{\}$ \tcp*{3-tuple min heap ordered by first item}
% $w\gets 0$, $w^*\gets f(r)$, $T\gets (\{r\},\emptyset)$\;
% $Q.\text{enqueue}((w^*, \text{null}, r))$\;
% \While{$Q\neq \emptyset$}
% {
%     $w_v, u, v \gets Q.dequeue()$\;\label{alg_pricing_line:dequeue}
%     \If{$v\notin S$}{
%         $S \gets S\cup \{v\}$\;
%         $w \gets w + w_v$\;
%         $F\gets F\cup\{e_{uv}\}$\;\label{alg_pricing_line:intermediate}
%         \If{$w < w^*$}
%         {
%             $w^* = w$\;\label{alg_pricing_line:update_st}
%             $T \gets$ subtree constructed from $F$\;\label{alg_pricing_line:update_ed}
%         }
%     }
%     \For{$u \gets G.neighbors(v)$}
%     {
%         \If{$u\notin S$}
%         {
%             $Q.\text{enqueue}((f(u)+g(e_{uv}), u, v))$\;\label{alg_pricing_line:enqueue}
%         }
%     }
% }
% \end{algorithm}


\subsection{Branching Rules}
After obtaining the fractional optimal solution of the MP, the BCP branches into two child nodes where the fractional optimum is not included in both.


==> conclusion.tex <==
\section{Conclusions and Future Work}
This paper discussed the time-optimal MCPP problem as a fundamental planning challenge for multi-robot systems.
The objective is to minimize the maximum coverage time for each robot (i.e., makespan).
Specifically, we considered the MCPP problem on a graph abstraction of the terrain to be coverage, which can be solved with a optimality ratio of 4 if its reduced RMMTC problem is solved to optimal.
We formulated the RMMTC problem as a MIP model for the first time, whereas most existing works focused on designing polynomial-time approximation algorithms to solve this NP-hard problem.
While the MIP model produces the optimal solutions for RMMTC, we designed two efficient suboptimal heuristics to reduce the model size if given limited runtime and memory.
Our proof demonstrates the correctness of the MIP model and the completeness of the reduced-size MIP models with the two heuristics.
We provided detailed experimental results, including the use of model optimization warm-startup and the comparisons with two state-of-the-art MCPP planners.
Our method is competitive which results in higher quality solutions at the cost of more runtime.
There are several future works based on our work.
First of all, specialized heuristics for instances with clustered root vertices can significantly improve the MIP-based planner, as discussed in the previous section.
Also, for relatively large RMMTC instances, the proposed MIP models cannot solve efficiently and thus can be insufficient to solve large-scale MCPP problems in an acceptable runtime limit.
One potential direction is to leverage data-driven methods to train a model to stitch or merge sub-solutions from relatively smaller instances decomposed from the original instance.
In addition, it is rather convenient to build variants of the MCPP problem based on the proposed MIP models; for example, the MCPP variants where the inter-robot collision avoidance or minimized turnings are considered.
% It is also rather convenient to consider the capacitated version of the MCPP problem based on the proposed models, where robots can only cover limited regions within one trip and then should return to the depot to recharge.

==> heur.tex <==
\section{Efficient Suboptimal Heuristics}
While the MIP model can produce optimal solutions for RMMTC instances given adequate runtime, the graph size of the MIP model becomes too overwhelming to handle given limited runtime and memory when.
We observe that in optimal solutions for RMMTC instances, each subtree would typically grow from a neighborhood around its root, which tends to be far away from the roots of other subtrees.
To this end, we propose two efficient suboptimal heuristics to reduce the size of the original MIP model based on this observation.
The intuition is as follows:
1) an inferior graph $H_{ij}$ is generated for the root $r_i$ with respect to root $r_j$, where the vertices from $H_i$ are not likely to be covered by the subtree rooted at $r_i$;
2) for each rooted subtree, a residual graph is generated by removing all sets of inferior graphs $H_{ij}$ on the original graph $G$;
3) the MIP model is solved on these residual graphs for every subtree without considering the whole graph $G$.
We describe the proposed two heuristics in detail in the following.
\begin{figure}[htb]
\centering
\begin{subfigure}[b]{0.49\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/heur_demo/parabolic.png}
\caption{Parabolic removal heuristics}
\end{subfigure}
\hfill
\begin{subfigure}[b]{0.48\linewidth}
\centering
\includegraphics[width=\linewidth]{figs/heur_demo/subgraph.png}
\caption{Subgraph removal heuristics}
\end{subfigure}
\caption{Proposed suboptimal heuristics on the root vertex (red star) to all other root vertices (colored circles). Black squares, black crosses, and black dots are obstacles, inferior graph vertices, and residual graph vertices, respectively.}
\label{fig:heur_demo}
\end{figure}

\subsection{Parabolic Removal Heuristics}
For each $i\in I$ and $j\in I/\{i\}$, we define a parabola $\Omega_{ij}: y'=(a_{ij}x')^2$ under an arbitrary Cartesian coordinate system $o(x', y')$, with the root vertex $r_j$ as its base and ray $r_i\rightarrow r_j$ as its symmetric axis.
The width $a_{ij}$ of $\Omega_{ij}$ is given by:
\begin{equation}\label{eqn:alpha}
a_{ij}=\alpha\cdot\sigma\left[d(r_j, c_{ij})/d({r_i, r_j})\right]
\end{equation}

In Eqn.~(\ref{eqn:alpha}), $\alpha\geq 0$ is a parameter to adjust the parabola width, and $d(\cdot,\cdot)$ is the shortest path distance between two vertices on graph $G$ with each edge weighted by $w_e$.
The boundary intersection vertex $c_{ij}$ is defined by $ \argmax_{v\in B}[d(r_i, v)-d(r_j, v)]$, where $B$ is the set of boundary vertices of graph $G$.
In a 4-way connected graph, $B$ is the set of vertices whose degrees are less than 4.
Such a design follows the aforementioned intuition, where the generated parabolic region $\Omega_{ij}$ is not likely to be covered for the subtree rooted at $r_i$, and $\Omega_{ij}$ becomes smaller when $r_i$ is close to $r_j$ or $r_j$ is close to the graph boundaries.
Note that when $\alpha=0$, the parabola is a straight line perpendicular to $r_i\rightarrow r_j$.
Fig.~\ref{fig:heur_demo}-(a) demonstrates how the parabola $\Omega_{ij}$ is generated and the resulting inferior and residual graphs.
Let the subgraph induced by the parabola be the inferior graphs $H_i$ for each $i\in I$, and we obtain the Parabolic Removal Heuristics (PRH).
For each $v\in V(H_i)$ and each $e\in E(H_i)$ where $i\in I$: 1) remove all the vertex variables $y^i_v$; 2) remove all the edge variables $x^i_e$; 3) remove all the flow variables $f^i_{e,u}$ and $f^i_{e,v}$.
\begin{algorithm}[t]
\DontPrintSemicolon
\caption{Connectivity-Check}\label{alg:cc}
\KwData{graph $G$=$(V,E)$, root $r_i\in R$, inferior graph $H_i$}
\KwResult{updated inferior graph $H_i$}
$C_r\gets $ connected component of $r_i$ in $H_i$\;
$\mathcal{C}\gets $ list of connected components of $H_i$\;
\For{$C \in \mathcal{C}/\{C_r\}$}
{
    $v\gets $ vertex of $C$ nearest to residual graph $G-H_i$\;
    $\pi\gets $ shortest path from $v$ to $r_i$\;
    $H_i\gets (V(H_i)/V(\pi), E(H_i)/E(\pi))$ 
}
\Return $H_i$\;
\end{algorithm}

During each removal of an inferior graph $H_i$, it might make the residual graph disconnected.
Therefore, after each removal corresponding to $H_i$, we adopt Alg.~\ref{alg:cc} for connectivity check to ensure the residual graph is connected.
Although the PRH applied on the original MIP model (MIP-PRH) does not ensure optimality, it does ensure completeness after the connectivity check.
We now give its proof of completeness as follows.
\begin{proof}
We need to prove that the solution space of the MIP-PRH still contains feasible $k$-rooted tree cover solutions after the corresponding variables in the parabolas are removed for each subtree.
In other words, the removed vertex variables for each subtree must be considered covered by other subtrees.
Without loss of generality, we consider the parabola $\Omega_{ij}$ with respect to some $r_i$ and $r_j$.
It is obvious that either $\Omega_{ij}\cap\Omega_j=\emptyset$ or $\Omega_{ij}\cap\Omega_j\neq\emptyset$.
For the first case, all removed vertices in $\Omega_{ij}$ are considered to be covered by the subtree rooted $r_j$.
According to the construction rules of the parabolas, it satisfies that $\Omega_{ij}\cap\Omega_{ji}=\emptyset$ for all $\alpha\geq 0$.
Therefore, the second case only holds if $\exists a\in I/\{i,j\}$ such that $\Omega_{ja}\cap\Omega_{ij}\neq\emptyset$, where we have the remaining area $\Omega_{ij,a}=\Omega_{ij}-\Omega_{ij}\cap\Omega_{ja}$ must satisfy either $\Omega_{ij,a}\cap\Omega_a=\emptyset$ or $\Omega_{ij,a}\cap\Omega_a\neq\emptyset$, and so on so forth.
Such a procedure will terminate when it loops over all roots of $R$ or $\Omega_{ij}\cap\Omega_{jb}=\emptyset$ with some root $r_b$.
Applying the same derivation on each parabola for $r_i\in R$, we have $\forall v\in\Omega_i, \exists j\in I, v\notin\Omega_j$.
Therefore, the MIP-PRH guarantees feasible solutions and thus is complete.
\end{proof}

\subsection{Subgraph Removal Heuristics}
Instead of the geometric way PRH uses to generate the inferior graphs, we propose a new one from the graph perspective, namely Subgraph Removal Heuristics (SRH).
Hence, we first adopt Alg.~\ref{alg:srh} to generate inferior graph $H_i$ to be removed for each $i\in I$, with the vertex size limit $b_{ij}$ of the Farthest-First-Search (FFS) tree given by:
\begin{equation}\label{eqn:beta}
b_{ij}=\left\lceil\beta\cdot|S_{ij}|\cdot\sigma\left[ d(r_i, r_j) / d(r_j, c_{ij}) \right]\right\rceil
\end{equation}
where $\beta$ is a parameter to adjust $b_{ij}$, and larger $b_{ij}$ results more areas to be removed and vice versa.
$S_{ij}$ is a set of vertices defined in line~\ref{alg:srh-Sij} of Alg.~\ref{alg:srh} where the FFS will be performed.
Given a root $r_i\in R$, the FFS is just a Breadth-First-Search rooted at $r_i$ with the queue prioritized by the distance from each vertex to $r_i$, which ensures the vertices farthest to $r_i$ included in the FFS tree at first.
Similar to PRH, the FFS tree of a subtree rooted at $r_i$ with respect to $r_j$ also follows the intuition as mentioned earlier, where the vertices of the FFS tree are not likely to be covered for the current rooted subtree.
In addition, the FFS tree size becomes smaller when $r_i$ is close to $r_j$ or $r_j$ is close to the graph boundaries.
Fig.~\ref{fig:heur_demo}-(b) shows the residual graph of $r_i$ after SRH, where the colored regions correspond to each $S_{ij}$.
Then similar to the PRH, for $i\in I$, we remove all vertex, edge, and flow variables corresponding to $H_i$.
We call the MIP model with SRH as MIP-SRH.

\begin{algorithm}
\DontPrintSemicolon
\caption{Subgraph-Removal-Heuristics}\label{alg:srh}
\KwData{graph $G$=$(V,E)$, root $r_i\in R$, limit $b_{ij}$}
\KwResult{inferior graph $H_i$ of $r_i$}
$H_i\gets (\emptyset, \emptyset)$\;
$B\gets$ the boundary vertices of graph $G$\;
\For{$r_j \in R/\{r_i\}$}
{
    $S_{ij} \gets \{v\,|\, d(r_i, v)>d(r_j, v), v\in V\}$\;\label{alg:srh-Sij}
    $c_{ij} \gets \argmax_{v\in B}[d(r_i, v)-d(r_j, v)]$\;
    $M\gets$ Farthest-First-Search tree rooted at $c_{ij}$ on the subgraph induced by $S_{ij}$ until $|V(M)|>b_{ij}$\;\label{alg:srh-bfs}
    $H_i\gets (V(H_i)\cup V(M), E(H_i)\cup E(M))$\;
}
\Return Connectivity-Check($G, r, H_i$)\;
\end{algorithm}

Same as the MIP-PRH, the MIP-SRH also does not ensure optimality but does ensure completeness.
The proof of its completeness follows the same derivation as the MIP-PRH, except for that $\Omega_{ij}\cap\Omega_{ji}=\emptyset$ for all $\alpha\geq 0$ is replaced by $H_{ij}\cap H_{ji}=\emptyset$ for all $\beta \geq 0$, since the FFS (line~\ref{alg:srh-bfs}) in Alg.~\ref{alg:srh} is performed in two disjoint subgraphs induced by $S_{ij}$ and $S_{ji}$.
Therefore we have the following theorem: for any removal heuristics with $H_{ij}\cap H_{ji}=\emptyset$, it satisfies that the reduced MIP model with the heuristics is complete.

\subsection{Efficiency-Optimality Tradeoff}
To verify the effectiveness of the two proposed heuristics, given a 10 minute runtime limit, we conduct an empirical study on MIP-PRH and MIP-SRH in several selected RMMTC instances as depicted in Fig.~\ref{fig:istc}.
The results are shown in Fig.~\ref{fig:heur_exp}, where the left big sub-figure shows the effectiveness of the variable removals with PRH and SRH, and the right small sub-figures shows the loss of optimality of PRH and SRH.
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/heur_exp}
\caption{Empirical study on MIP-PRH and MIP-SRH. In each sub-figure, MIP-PRH and MIP-SRH are plotted with a shared y-axis, where MIP-PRH (crosses and dashed lines) use the top x-axis with different $\alpha$ values, MIP-SRH (circles and solid lines) use the bottom x-axis with different $\beta$ values. The original MIP models are the rightmost points with $\alpha$=$\infty$ and $\beta$=$0$.
The left big sub-figure shows the number of variables of each model, and the right small sub-figures show the gaps (10 minutes runtime limits) between the obtained lower bounds of MIP-PRH and MIP-SRH models with the original MIP model.}
\label{fig:heur_exp}
\end{figure}

Empirically, we found that both PRH and SRH can effectively reduce the MIP model variables by an average of $42.8\%$ for PRH and $50.3\%$ for SRH, with an average loss of optimality of $2.86\%$ for PRH and $12.7\%$ for SRH.
Generally speaking, SRH is more robust than PRH since SRH can better generate inferior graphs with the consideration of the graph structures, which can be observed from the experimental evaluations in Sec.~\ref{sec:exp}.
For the parameter choosing in consideration of the efficiency-optimality tradeoff, it is recommended to select a smaller $\alpha$ for PRH or a larger $\beta$ for SRH to obtain a smaller MIP model if the runtime or memory is heavily limited, whereas a larger $\alpha$ or a smaller $\beta$ to preserve optimality if given more runtime and memory.


==> hier.tex <==
\section{Hierarchical Large-scale Planner}
Although the model sizes of MIP-PRH and MIP-SRH can be greatly reduced compared with the original MIP model, it is still not applicable for very large-scale graphs (e.g., field terrains in~\cite{tang2021mstc}), where the numbers of vertices and edges are too overwhelming in considerations of memory and runtime limitations.
Hence we aim to build a hierarchical scheme that first coarsen the original graph and solve a reformulated MIP model on the coarsen graph, then uncoarsen the solution to recover the solution on the original graph.

\subsection{Graph Coarsening}
Given the graph $G=(V,E)$ of an RMMTC instance, we denote its coarsened graph as $G_c=(V_c, E_c)$.
As shown in Fig.\ref{fig:graph_coarsen}, we adopt three graph coarsening methods to construct $G_c$, namely Light-Edge-Matching (LEM)~\cite{karypis1998fast}, Random-Contraction (RC) and Uniform-Contraction (UC).
\begin{figure}[htp]
\centering
\includegraphics[width=\linewidth]{figs/graph_coarsen.png}
\caption{Graph coarsening on the \textit{Reg. Grid \#2} instance~\cite{tang2021mstc}.}
\label{fig:graph_coarsen}
\end{figure}
For the LEM, \textit{Maximal Matching} are first found in a greedy fashion, then edges and vertices in each matching are contracted into a new vertex, with new edges connecting the contracted vertex and vertices outside the matching.
For the RC, BFS is performed on a uncontracted vertex via random sampling to contract the uncontracted vertices from the BFS tree.
For the UC, grid-like uniformly neighboring vertices are contracted into a new vertex, with new edges connecting the contracted vertex and vertices outside the neighborhood.

\subsection{Problem Reformulation}
Given a coarsened graph $G_c$ of $G$, we denote the corresponding vertex contraction mapping as $\delta:V_c\mapsto \mathcal{V}\subset\mathbb{P}(V)$, where $\mathbb{P}(V)$ is the power set of $V$.
Based on the original MIP model described in Eqn.~(\ref{eqn:obj})-(\ref{cstr:y_def}), we need to reformulate it for the hierarchical planner with a new binary variable $\textbf{z}=\{z^i_v\}^{i\in I}_{v\in V_c}\in\{0,1\}$ representing the agent $i$ covers vertices in $\delta(v)$ if $z_v^i=1$ otherwise do not.
Although most of the constraints can be easily rewritten by replacing each $V$ with $V_c$ and $E$ with $E_c$, the \textit{makespan} and \textit{cover} constraints need to be stressed with special reformulations in the following content.
\begin{figure}[htp]
\centering
\includegraphics[width=0.67\linewidth]{figs/coarsen_graph_local_view.png}
\caption{Local view of a coarsen graph. For each contracted vertex $v\in V_c$, the grey colored region is the corresponding vertex set $\delta(v)$, where the red vertex is the central vertex and the dashed edges are the MST $M_v$. The red edges are the shortest paths $\pi_{uv}$ for each neighboring $u, v\in V_c$.}
\label{fig:coarsen_graph_local_view}
\end{figure}

\subsubsection{Makespan}
The \textit{makespan} constraints in Eqn.~(\ref{cstr:makespan}) should be rewritten as below:
\begin{align}
\sum_{e\in E_c}w_e x_e^i + \sum_{v\in V_c}w(M_v)z_v \leq\tau, \quad\quad\forall i\in I
\end{align}
where $\pi_{uv}$ is the shortest path from $\delta(u)$ to $\delta(v)$, and $M_u$ is the \textit{Minimum Spanning Tree} (MST) of the subgraph of $G$ induced by $\delta(u)$.
For convenience, we define $\pi_{uv}$ to be the shortest path between two central vertices from $\delta(u)$ and $\delta(v)$ respectively, where the central vertex of a vertex set is just the geometry center of all vertices from the set.
Fig.~\ref{fig:coarsen_graph_local_view} depicts the local view of two edges connecting three contracted vertices in a coarsened graph $G_c$.

\subsubsection{Cover}
With the new variable $\textbf{z}$ introduced, the \textit{cover} constraint in Eqn.~(\ref{cstr:cover}) should be rewritten as:
\begin{align}
\sum_{i\in I}z_v^i = 1, \quad\quad\quad\forall v\in V_c
\end{align}
To enforce the correctness of each $z^i_v, i\in I, v\in V_c$, we also need to add the constraints $z^i_v \leq y^i_v$ to the model.

\subsection{Solution Recover}




==> intro.tex <==
\section{Introduction}
Coverage Path Planning (CPP) is the problem of finding an optimal path for a robot to traverse over an terrain of interest to completely cover its all regions.
For example, the terrain can be indoor environments covered by vacuum cleaning robots~\cite{bormann2018indoor} or outdoor fields covered by unmanned aerial vehicles~\cite{lin2009uav}.
Over the past few decades, significant attention has been given to CPP in the robotics community, leading to a considerable amount of research focused on addressing this problem~\cite{galceran2013survey}.
Multi-Robot Coverage Path Planning (MCPP) is an extension of CPP, which involves coordinating the paths of multiple robots to achieve complete coverage of the given terrain, thus improving the coverage task efficiency and system robustness.
Therefore, MCPP plays a significant role in various applications such as search and rescue~\cite{song2022multi}, environmental monitoring~\cite{collins2021scalable}, and mapping~\cite{azpurua2018multi}.
Developing efficient and robust MCPP algorithms is essential to enable widespread deployment of multi-robot systems in robotics applications.

One of the main challenges in MCPP is to design an algorithm that can effectively distribute the robots over the terrain to be covered while avoiding collisions with static obstacles.
It requires considering factors such as the terrain's traversability, the robots' mobility, and the availability of communication between the robots.
Additionally, the problem becomes increasingly complex as the number of robots increases, as the algorithm must consider more potential paths and interactions between the robots.
Another challenge in MCPP is to ensure that the coverage is complete, that is, all regions of the terrain are covered, which can be challenging to achieve without sacrificing efficiency or incurring high computational costs.

In this paper, we consider the fundamental challenge of time-optimal multi-robot planning in MCPP, where the maximal coverage time of all robots (i.e., makespan) is minimized.
Specifically, we focus on MCPP applications like agriculture and environment monitoring, where the path execution time is assumed to be an order of magnitude higher than the planning time.
In other words, the solution quality matters more than the planning runtime.
Under the above assumption,  offline planning is commonly used to solve the MCPP problems without the need of inter-robot communications.
To this end, we leverage the similar problem modeling from~\cite{gabriely2001spanning, gabriely2002spiral, zheng2005multi, zheng2007robot, zheng2010multirobot} to solve the problem, where the terrain to be covered is abstracted as a weighted or unweighted graph, and the makespan is evaluated by the weights of a set of graph edges (i.e., the coverage path).
We conclude our main contributions as below:
\begin{enumerate}
\item We propose a Mixed Integer Programming (MIP) model for the Rooted Min-Max Tree Cover (RMMTC) problem and prove its correctness, which is used to solve its corresponding MCPP problem with an optimality ratio of 4. We prove the correctness of the proposed MIP model.
\item Based on the proposed MIP model, we design two efficient suboptimal heuristics, namely Parabolic Removal Heuristics and Subgraph Removal Heuristics, to reduce the MIP model size, which efficiently solves RMMTC instances with a configurable loss of optimality. We prove the completeness of the two reduced-size MIP models. 
\item We open-sourced our method to the robotics community, and provide thorough experimental results on the use of model optimization warm-startup and the performance comparisons between state-of-the-art planners, namely MFC and MSTC$^*$.
Our MIP-based planners results in higher quality solutions with the cost of more runtime.
\end{enumerate}

==> problem.old.tex <==
\newcommand{\Sngb}[1]{\mathcal{N}(#1)}

\section{Problem Formulation}
Consider an undirected graph $G = (V, E)$, where $V = \{1, ..., n\}$ is the set of $n$ vertices.
There is a set of root vertices $R\subseteq V$.
For each vertex $v\in V$, we denote the set of its neighboring nodes as $\Sngb{v}$.
Each edge $(u, v) \in E, \forall u, v \in V$ has an associated cost $c_{uv}$.
Given a parameter $k$ and denote a set $I=\{1, 2, ..., k\}$, a feasible solution of the RMMTC problem is a set of $k$ subtrees $\{T_{i}\}_{i\in I}$ such that: (a) each $T_i$ must be rooted at vertex $r\in R$, and (b) each vertex $v\in V$ is covered or included in at least one subtree.

We define binary variables $\textbf{x} = [x^i_{uv}]^T$, where $x^i_{uv}\in\{0, 1\}$ takes value $1$ if edge $(u, v) \in E$ is included in the $i$-th subtree $T_i$ and $0$ otherwise for each $i\in I$.
Next, we define binary variables $\textbf{y} = [y^i_{v}]^T$, where $y^i_{v}\in\{0, 1\}$ takes value $1$ if vertex $v \in V$ is covered in the $i$-th subtree $T_i$ and $0$ otherwise for each $i\in I$.
Let $\tau$ represent the maximum cost of all the subtrees, we formulate a Mixed Integer Program (MIP) for the \textbf{RMMTC (\textcolor{blue}{MMTC w/ constraints (\ref{cstr1:rooted}) removed)}} as follows:
\begin{align}
\label{eqn:obj_1}\textbf{(MIP)}&\quad\displaystyle{\minimize_{\textbf{x}, \textbf{y}, \tau}\quad\tau}&\\
\label{cstr1:makespan}\text{s.t.}&\sum_{(u, v) \in E} c_{uv} x_{uv}^i \leq \tau, &\forall i\in I\\
\label{cstr1:cover}&\sum_{i\in I} y_{v}^i\geq 1, &\forall v \in V\\
\label{cstr1:rooted}&y^i_{r_i} = 1, 
&\forall i\in I\\
\label{cstr1:subtree_conn}&\sum_{v\in V} y_{v}^i = 1+\sum_{(u, v)\in E} x_{uv}^i, &\forall i\in I\\
\label{cstr1:subtour_elim}&\textcolor{red}{\sum_{(u,v)\in E, u,v\in S} x^i_{uv}\leq |S|-1,} &\textcolor{red}{\forall S\subseteq V, \forall i\in I}
\end{align}
\vspace{-12pt}
\begin{flalign}
\label{cstr1:y_of_x} \hspace{26pt} x^i_{e}\leq y^i_v,  \quad\quad\quad\quad&\forall v\in V, \forall e\in E, e\sim v, \forall i\in I
\end{flalign}
where constraints (\ref{cstr1:makespan}) ensure that $\tau$ equals to the maximum cost of all the subtrees, which is minimized in the objective function (\ref{eqn:obj_1});
constraints (\ref{cstr1:cover}) ensure the coverage of all vertices, that is, each vertex is included by an arbitrary subtree for at least once;
\textcolor{blue}{constraints (\ref{cstr1:rooted}) ensure that each subtree must include an arbitrary root from the given set of root vertices;}
constraints (\ref{cstr1:subtree_conn}) and (\ref{cstr1:subtour_elim})  enforce that each subtree has only one connected component without cycles;
constraints (\ref{cstr1:y_of_x}) enforce the relationship between $y^i_v$ and $x^i_{uv}$ by definition.


==> problem.tex <==
\section{Problem Formulation}

\subsection{Graph-based Spanning Tree Coverage}\label{subsec:stc}
Following~\cite{zheng2005multi, zheng2007robot, zheng2010multirobot}, we consider the coverage problem for both weighted and unweighted terrains with the graph-based Spanning Tree Coverage (STC) \cite{gabriely2001spanning, gabriely2002spiral}, where the terrain is represented by a graph $\mathcal{G}$ and the robot(s) should start from and end at a given initial vertex of $\mathcal{G}$.
For convenience, we restrict ourselves to MCPP with weighted terrain, that is, each vertex $v$ of $\mathcal{G}$ has an associating weight $w(v)$, since we can simply assign a uniform weight of $1$ for each vertex of $\mathcal{G}$ for the cases of unweighted terrain.
Given a terrain graph $\mathcal{G}$ as shown in Fig.~\ref{fig:spanning_tree_coverage}-(a) and (b), each vertex of $\mathcal{G}$ is decomposed into four smaller adjacent vertices.
We denote the graph consisting of the decomposed vertices as $\mathcal{H}$, where each vertex of $\mathcal{H}$ needs to be visited by at least one robot for the complete coverage.
Then, for every vertex $v$ of $\mathcal{H}$ resulting from the decomposition of the vertex $u$ of $\mathcal{G}$, we assign $v$ with a weight $w(v)=w(u)/4$.
\begin{figure}[b]
\centering
\includegraphics[width=\linewidth]{figs/spanning_tree_coverage}
\caption{Graph-based STC in the instance from~\cite{zheng2010multirobot, tang2021mstc}: (a) local view of STC modeling of a weighted terrain to be covered; (b) black squares, color-filled markers, and hollowed circles represent obstacles, vertices of $\mathcal{G}$, and vertices of $\mathcal{H}$, respectively; (c)(d) thin lines and thick lines represent the rooted subtrees in $\mathcal{G}$ and the resulting coverage paths in $\mathcal{H}$.}
\label{fig:spanning_tree_coverage}
\end{figure}
For both $\mathcal{G}$ and $\mathcal{H}$, an edge $(u, v)$ is connected for each pair of vertically or horizontally adjacent vertices, where the edge weight is defined as $\left(w(u)+w(v)\right)/2$.
The coverage time of a valid complete coverage path $\pi=(v_1, v_2, ..., v_{|\pi|})$ in $\mathcal{H}$ is thereby defined as $t(\pi)=\sum_{i=1}^{|\pi|}\left[\left(w(v_{i})+w(v_{i+1})\right)/2\right]$. ($v_{|\pi|+1}=v_1$ is the assigned initial vertex of the robot.)
For CPP on the constructed graphs $\mathcal{G}$ and $\mathcal{H}$ as depicted in Fig.~\ref{fig:spanning_tree_coverage}-(c), STC works by circumnavigating an arbitrary spanning tree of $\mathcal{G}$, which generates a coverage path in $\mathcal{H}$ by letting the robot always moving along the right side of the spanning edges.
Since $\pi$ visits (i.e., enters and leaves) each vertex of $\mathcal{H}$ at least once, we further have $t(\pi)=\sum_{i=1}^{|\pi|}w(v_{i})$, which is at least the sum of the weights of all vertices in $\mathcal{H}$ (also equals to the sum of weights of all vertices in $\mathcal{G}$).
Note that STC is guaranteed to generate a coverage path in $\mathcal{H}$ where each vertex in $\mathcal{H}$ is visited exactly once.
It follows that for the CPP problem, STC is time-optimal using arbitrary spanning tree of $\mathcal{G}$ in unweighted terrains~\cite{gabriely2001spanning}, and time-optimal using the minimum spanning tree of $\mathcal{G}$ in weighted terrains~\cite{zheng2007robot}.

For MCPP as shown in Fig.~\ref{fig:spanning_tree_coverage}-(d), STC is extended for multi-robot scenarios~\cite{zheng2005multi, zheng2007robot, zheng2010multirobot} by first building multiple subtrees that jointly cover all the vertices of $\mathcal{G}$, and then using STC to generate coverage path in $\mathcal{H}$ on each subtree rooted of $\mathcal{G}$ at the given initial vertex for each robot.
As demonstrated in Theorem 4 of~\cite{zheng2007robot}, based on the time-optimality of STC, the above extended STC solves MCPP with an optimality ratio of 4 if the set of rooted subtrees is optimal with a minimized makespan of subtree weights.
As finding such an optimal set of rooted subtrees on $\mathcal{G}$ is proven to be NP-hard for either unweighted terrains~\cite{even2004min} or weighted terrains~\cite{zheng2010multirobot}, MFC~\cite{zheng2005multi, zheng2007robot, zheng2010multirobot} adopts RTC~\cite{even2004min} to solve it approximately.
This inspires us to find the optimal set of rooted subtrees on $\mathcal{G}$ via an exact approach, which currently does not exist to the best of our knowledge.
We call such a problem as the Rooted Min-Max Tree Cover (RMMTC) problem, which is also known as the $R$-Rooted Tree Cover problem~\cite{even2004min} or the Multi-Rooted Subtree Cover problem~\cite{nagamochi2007approximating} in the operations research literature.

\subsection{The Rooted Min-Max Tree Cover Problem}
Consider an undirected graph $G = (V, E)$, where $V = \{1, ..., n\}$ is the set of $n$ vertices and $E$ is the set of $m$ edges.
Each edge $e=(u, v) \in E, u,v \in V$ has an associated weight $w_e$, which is the average of the terrain weights of $u$ and $v$ as defined in Sec.~\ref{subsec:stc}.
Given a set of root vertices $R=\{r_i\}_{i\in I}\subseteq V$ where $I=\{1, 2, ..., k\}$ is an index set, a feasible solution for RMMTC is a set of $k$ subtrees $\{T_{i}\}_{i\in I}$ such that: a) each $T_i$ must be rooted at an arbitrary root vertex $r\in R$, and b) each vertex $v\in V$ is included in at least one subtree.
Define the weight of subtree $T_i$ as $w(T_i)=\sum_{e\in T_i}w_e$, the objective of RMMTC is to find the optimal set of subtrees:
\begin{align}
\{T_i\}_{i\in I}^* = \argmin_{T_1,T_2,...,T_k} \max\{w(T_1), w(T_2), ..., w(T_k)\}
\end{align}

To formulate the RMMTC problem, we first define two sets of binary variables $\textbf{x} = \{x^i_{e}\}_{e\in E}^{i\in I}$ and $ \textbf{y} = \{y^i_{v}\}_{v\in V}^{i\in I}$, where $x^i_{e}, y^i_v\in\{0, 1\}$ take value $1$ if $e$ or $v$ are included in the $i$-th subtree $T_i$ and $0$ otherwise, respectively.
We then define a set of continuous variables $\textbf{f} = \{f^i_{e,u}, f^i_{e,v}\}_{e\in E}^{i\in I}$, where $f^i_{e,u}, f^i_{e,v}\in\mathbb{R}^+$ represent the flows sent by the edge $e=(u,v)$ to vertex $u$ and vertex $v$, respectively.
Let $\tau$ represent the maximum weight among all the subtrees (i.e., makespan), and $e\sim v$ denotes $v$ as one of the endpoint vertices of $e$, we then formulate a MIP model for the RMMTC problem as follows:
\begin{align}
\label{eqn:obj}\textbf{(MIP)}&\quad\displaystyle{\minimize_{\textbf{x}, \textbf{y}, \textbf{f}, \tau}\quad\tau} &\\
\label{cstr:makespan}\text{s.t.}\quad&\sum_{e \in E} w_{e} x_{e}^i \leq \tau, &\forall i\in I \\
\label{cstr:cover}&\sum_{i\in I} y_{v}^i\geq 1, &\forall v \in V\\
\label{cstr:rooted}&y^i_{r_i} = 1, &\forall i\in I\\
\label{cstr:tree_def}&\sum_{v\in V} y_{v}^i = 1+\sum_{e\in E} x_{e}^i, &\forall i\in I\\
\label{cstr:acyclic_1} \quad\quad&f_{e,u}^i+f_{e,v}^i=x_{e}^i, &\forall e=(u,v)\in E, \forall i\in I\\
\label{cstr:acyclic_2} \quad\quad&\sum_{\substack{e\in E\\ e\sim v}}f_{e,v}^i\leq 1- \frac{1}{n}, &\forall v\in V, \forall i\in I
\end{align}
\vspace{-12pt}
\begin{flalign}
\label{cstr:y_def} \hspace{26pt} x^i_{e}\leq y^i_v,  \quad\quad\quad\quad&\forall v\in V, \forall e\in E, e\sim v, \forall i\in I
\end{flalign}
\vspace{-16pt}
\begin{flalign}
\hspace{26pt} x^i_{e}, y^i_v\in\{0, 1\},  \quad\quad\quad\quad&\forall v\in V, \forall e\in E, \forall i\in I
\end{flalign}
\vspace{-16pt}
\begin{flalign}
\hspace{24pt} f^i_{e,u}, f^i_{e,v}, \tau\in\mathbb{R}^+, \quad\quad&\forall e=(u, v)\in E, \forall i\in I
\end{flalign}

We group the constraints of the above MIP model as below:
\begin{enumerate}
\item \textit{Makespan}:
Eqn.~(\ref{cstr:makespan}) ensures that $\tau$ equals to the maximum weight among all the subtrees, which is minimized in the objective function in Eqn.~(\ref{eqn:obj});
\item \textit{Cover}:
Eqn.~(\ref{cstr:cover}) enforces that each vertex is included in an arbitrary subtree at least once;
\item \textit{Rooted}: 
Eqn.~(\ref{cstr:rooted}) enforces that each subtree must be rooted at vertex $r_i\in R$;
\item \textit{Tree}:
Eqn.~(\ref{cstr:tree_def}) ensures that each subtree is either a single tree or a forest with cycles in some of its trees, whereas
Eqn.~(\ref{cstr:acyclic_1}) and (\ref{cstr:acyclic_2}) eliminate any cycles in each subtree. Together they enforce each subtree is one single tree.
\end{enumerate}

Besides the above group constraints, Eqn.~(\ref{cstr:y_def}) enforces the consistency between edge variables $x^i_e$ and vertex variables $y^i_v$ for each subtree, which implies that the vertex is included if and only if at least one of its incident edges is included.
While the other group constraints are straightforward to verify, the
\textit{Tree} group constraint borrowed from~\cite{cohen2019several, althaus2014algorithms} is not self-evident for our MIP formulation.
To this end, we prove each subtree is one single tree if the \textit{Tree} group constraint hold.
\begin{proof}
For the \textit{Tree} group constraints consisted of Eqn.~(\ref{cstr:tree_def}), (\ref{cstr:acyclic_1}), and (\ref{cstr:acyclic_2}), we denote their sub-components corresponding to an arbitrary $i\in I$ as Eqn.~(\ref{cstr:tree_def}-$i$), (\ref{cstr:acyclic_1}-$i$), and (\ref{cstr:acyclic_2}-$i$), respectively.
Given Eqn.~(\ref{cstr:tree_def}-$i$), we can first easily verify for subtree $T_i$, it is either a tree or a forest with $C-1$ cycles in its $C$ trees.
We now prove for $T_i$, the latter case does not hold as Eqn.~(\ref{cstr:acyclic_1}-$i$) and (\ref{cstr:acyclic_2}-$i$) would eliminate any potential cycles.
\begin{figure}[htp]
\centering
\includegraphics[width=0.48\linewidth]{figs/tree_proof}
\caption{Connected sub-component with a potential cycle.}
\label{fig:tree_proof}
\end{figure}

As shown in Fig.~\ref{fig:tree_proof}, without loss of generality, we assume there is a connected sub-component $S$ belonging to one of the trees from $T_i$, where $V(S)=\{a_j\}_{ j=1,2...,s}\subsetneq V(T_i)$ and $E(S)=\{(a_j, a_{j+1})\}_{ j=1,2...,s-1}\subsetneq E(T_i)$ are included.
In addition, we assume edge $e_c=(a_1, a_s)\in E(G)$ would add a potential cycle to $T_i$ if $e_c\in E(S)$.
By summing up Eqn.~(\ref{cstr:acyclic_1}-$i$) for all edges $e\in\{e_c\}\cup E(S)$, we have:
\begin{align}\label{eqn:sum_cstr_acyclic_1}
(f^i_{e_c, a_1} + f^i_{e_c, a_s})+\sum_{e\in E(S)}\left(f^i_{e, u}+f^i_{e, v}\right)=x^i_{e_c} + s-1
\end{align}

Denote edge set $F_i=E(T_i)/E(S)/\{e_c\}$, by summing up Eqn.~(\ref{cstr:acyclic_2}-$i$) for all vertices $v\in V(S)$, we have:
\begin{align*}
&\sum_{v\in V(S)}\sum_{\substack{e\in E\\e\sim v}} f^i_{e, v}\nonumber\\
=\;& (f^i_{e_c, a_1} + f^i_{e_c, a_s})+\sum_{e\in E(S)}(f^i_{e, u}+f^i_{e, v})+
\sum_{v\in V(S)}\sum_{\substack{e\in F_i\\ e\sim v}} f^i_{e, v}\nonumber\\
\leq\; & s\cdot(1-\dfrac{1}{n})
\end{align*}
combining with Eqn.~(\ref{eqn:sum_cstr_acyclic_1}), we get the following inequality:
\begin{align}\label{eqn:tree_proof_eq}
x^i_{e_c}\leq 1 - \dfrac{s}{n} - \sum_{v\in V(S)}\sum_{\substack{e\in F_i\\e\sim v}} f^i_{e, v} < 1
\end{align}
thus $x^i_{e_c}\in\{0,1\}$ can only be $0$.
This implies there cannot be any cycles in subtree $T_i$, 
and since $T_i$ is either a tree or a forest with cycles, $T_i$ now must be a tree.
Thus we have proved $\forall i\in I$, $T_i$ is a tree if the \textit{Tree} group constraint holds.
\end{proof}

The above proposed MIP model has $\mathcal{O}\left(k(n+3m)\right)$ variables and $\mathcal{O}\left(n+k(3+m+n)+kn\bar{d}\right)$ constraints, where $\bar{d}$ is the average degree of vertices depending on the structure of the input graph.
In this paper, all RMMTC instances are considered to be 4-way connected graphs, meaning that $\bar{d}=4$.


==> related_work.tex <==
\section{Related Work}
\subsection{Single-Robot and Multi-Robot Coverage Path Planning}
The CPP aims to plan a path for a robot to completely cover the given terrain, which is a well-studied single-robot planning problem in the literature.
We refer interested readers to the extensive surveys~\cite{choset2001coverage, galceran2013survey} on CPP.
For the MCPP problem, most algorithms are built upon existing CPP algorithms by first decomposing the terrain to be covered to multiple sub-areas with coverage paths, then assigning the paths to multiple robots.
In general, both CPP and MCPP algorithms can be categorized into decomposition-based and graph-based.
The decomposition-based methods~\cite{acar2002morse, rekleitis2008efficient, karapetyan2017efficient} first geometrically decompose the terrain and then generate back-and-forth coverage paths (e.g., boustrophedon) on each sub-area. In contrast, the graph-based methods~\cite{gabriely2002spiral, hazon2005redundancy, kapoutsis2017darp} proceed on the graph structure of the terrain to be covered, which we will discuss in detail in the next paragraph.
More recently, several learning-based planners~\cite{theile2020uav, lakshmanan2020complete, tang2022learning} are also proposed to solve some application-specific coverage problems, where the uncertainties of robots and environment are a major consideration for the problem.

One of the well-known methods to solve the coverage problem is the graph-based \textit{spanning tree coverage}~\cite{gabriely2001spanning}, where the terrain to be covered is abstracted into uniformly distributed vertices sampled on the given bounded region, and robots are allowed to traverse along adjacent vertices.
By choosing the vertex sampling distance to ensure every region can be swept by traversing between adjacent vertices, the coverage problem can be solved by covering all the vertices of the graph.
Although the single-robot coverage problem can be solved optimally in unweighted terrains~\cite{gabriely2001spanning} and near-optimally in weighted terrains~\cite{zheng2007robot} in polynomial time using the Spanning Tree Coverage (STC) algorithm~\cite{gabriely2001spanning}, the multi-robot coverage problem with STC has been proved to be NP-complete~\cite{zheng2010multirobot}.
Therefore, most works focus on designing polynomial-time approximation algorithms.
Hazon et al. first proposed the Multi-Robot Spanning Tree Coverage (MSTC) algorithm~\cite{hazon2005redundancy} based on the single-robot STC algorithm to the multi-robot scenario, which split the STC path into multiple segments based on the initial location of each robot and then assigns them to the robots.
The idea behind MSTC was further improved by constructing better spanning trees to generate better STC path~\cite{agmon2006constructing}, by finding balanced cut points on the STC path~\cite{tang2021mstc}.
It was extended to support scenarios with fault-tolerance~\cite{sun2021ft} and minimized turnings~\cite{lu2022tmstc}.
Unlike directly splitting the STC path, Zheng et al. proposed Multi-Robot Forest Coverage (MFC)~\cite{zheng2005multi, zheng2007robot, zheng2010multirobot}, which extends the Rooted Tree Cover (RTC) algorithm~\cite{even2004min} to generate multiple rooted subtrees to cover all vertices of the input graph, and then generate coverage path by using STC on each subtree.

\subsection{Integer Programming for Multi-Robot Planning}
Integer Programming (IP) is a mathematical optimization technique used to solve problems that involve discrete variables under several problem-specific constraints.
Mixed Integer Programming (MIP) is a special case of IP when the problem model also involves continuous variables.
Given adequate time, both IP and MIP models can be solved to optimum via branch-and-bound methods on top of linear relaxation of the model, and they have been used extensively in multi-robot planning.
Han et al.~\cite{han2019integer} proposed a general IP framework to solve several path-based optimization problems, including multi-robot path planning and multi-robot minimum constraint removal.
Lam et al.~\cite{lam2022branch} proposed a Branch-and-Cut-and-Price framework based on an IP model to efficiently solve the multi-agent path finding problem, where different robots must traverse from an initial location to a goal location.
Asfora et al.~\cite{asfora2020mixed} presented a MIP model to tackle the multi-robot efficient
search path planning problem, where multiple robots must capture a moving target within a given time limit.
Lippi et al.~\cite{lippi2021mixed} formulated a MIP model to solve the task allocation problem for a system with humans and multiple robots.
Despite MIP and IP having been shown to be effective in finding optimal solutions for a wide range of problems, as the problem size grows, the computational complexity of the MIP solver increases exponentially, making it challenging to solve large-scale problems in limited runtime.
Therefore, many existing works focus on designing efficient heuristics based on the MIP or IP framework~\cite{yu2016optimal, guo2021spatial}.
